Tailoring Self-Supervision for Supervised Learning

Recently, it is shown that deploying a proper self-supervision is a prospective way to enhance the performance of supervised learning. Yet, the benefits of self-supervision are not fully exploited as previous pretext tasks are specialized for unsupervised representation learning. To this end, we begin by presenting three desirable properties for such auxiliary tasks to assist the supervised objective. First, the tasks need to guide the model to learn rich features. Second, the transformations involved in the self-supervision should not significantly alter the training distribution. Third, the tasks are preferred to be light and generic for high applicability to prior arts. Subsequently, to show how existing pretext tasks can fulfill these and be tailored for supervised learning, we propose a simple auxiliary self-supervision task, predicting localizable rotation (LoRot). Our exhaustive experiments validate the merits of LoRot as a pretext task tailored for supervised learning in terms of robustness and generalization capability. Our code is available at https://github.com/wjun0830/Localizable-Rotation.

==> _6_limitation.tex <==
\subsection{Limitation, Discussion}
% Hereby, we point out limitations.
First, as mentioned in Sec. \ref{subsection:OODExperiments}, the merits of LoRot are not fully exploited in simple datasets with plain backgrounds, e.g., SVHN.
It is because there is no difference when a small patch is rotated against the plain background.
% It also applies when the average size of the object is tiny so that rotated patches do not contain any object parts most of the time.
It is also the case when the size of the object is tiny so that rotated patches do not contain any object parts most of the time.
% applies는 안맞는말인거 같은데. average size도 위 context에서는 갑자기 나오는거 같고.
In this context, practitioners should be aware of the average size of the object or background constituting the dataset when applying LoRot to other models.

Still, as there aren't many cases where the real image has a plain background, and LoRot is an effective, efficient, and easy-to-implement strategy over previous pretext tasks, we believe the strength of LoRot outweighs the limitation.

